Comparing Workflow Application Designs for High Resolution Satellite Image Analysis

Very High Resolution satellite and aerial imagery are used to monitor and conduct large scale surveys of ecological systems. Convolutional Neural Networks have successfully been employed to analyze such imagery to detect large animals and salient features. As the datasets increase in volume and number of images, utilizing High Performance Computing resources becomes necessary. In this paper, we investigate three task-parallel, data-driven workflow designs to support imagery analysis pipelines with heterogeneous tasks on HPC. We analyze the capabilities of each design when processing datasets from two use cases for a total of 4,672 satellite and aerial images, and 8.35 TB of data. We experimentally model the execution time of the tasks of the image processing pipelines. We perform experiments to characterize the resource utilization, total time to completion, and overheads of each design. Based on the model, overhead and utilization analysis, we show which design is best suited to scientific pipelines with similar characteristics.

==> performances_characterization.tex <==
% !TEX root = main.tex

In this section, we use three metrics to characterize and compare the
performance of CPU-SIFT, CUDA-SIFT, and GPU-SIFT\@: throughput, memory
consumption and matching accuracy. We match single pairs of increasingly
large GeoTIFF images (source and target), measuring how many MB are processed
by the CPU or GPU per second, how much memory the matching of the images
required and how accurate such a matching was.

We performed all our experiments on the XSEDE Bridges
supercomputer~\cite{nystrom2015bridges}. Bridges offers 32 nodes with 2 Tesla
P100 GPUs and 32~GB of GPU-dedicated memory, and 2 16-cores Intel Broadwell
E5--2683 CPUs with 128~GB of RAM\@. We used RADICAL-Pilot~\cite{merzky2018using}
to manage the execution of our experiment workloads on Bridges. For all the
experiments, we use a single GeoTIFF image of $\approx$845~MB, tailed into four
predefined sizes: 90, 180, 360, 720~MB\@. We then match two copies of the same
tail for each size, using each SIFT implementation.

% ---------------------------------------------------------------------------
\subsection{Throughput}

We measure the throughput of CPU-SIFT, CUDA-SIFT, and GPU-SIFT in MB/s when
processing the same pair of 90, 180, 360 and 720~MB images. %As seen
%in~\S\ref{ssec:increase_alloc},
CPU-SIFT and CUDA-SIFT can analyze one pair
of images per CPU/GPU, while GPU-SIFT can use CUDA MPS to analyze two pairs
of images per GPU\@. Consistently, in our experiments we concurrently execute
two CPU-SIFT on two CPUs, two CUDA-SIFT on two GPUs and one GPU-SIFT on one
GPU\@.

Fig.~\ref{fig:throughout} shows that CPU-SIFT (red) has the lowest throughput
with a value of 54.38~MB/sec. This is due to CPU-SIFT programming model:
CPU-SIFT uses one core per CPU to process and match two images. As a result,
CPU-SIFT cannot leverage the parallelism supported by multi-core architecture
to increase throughput.

CUDA-SIFT (dark green) has a throughput almost six times higher than
CPU-SIFT, with a value of 244.44~MB/sec. Different from CPU-SIFT, CUDA-SIFT
uses the CUDA framework to load balance calculations across the cores of the
GPU device. Nonetheless, note that with the given images, CUDA-SIFT uses only
up to 1,658 of the 3,584 CUDA cores available on the Nvidia P100 GPU devices
of our experiments. There are not enough data to process to saturate the GPU
cores.

GPU-SIFT (light green) has the highest throughput among the three SIFT
implementations, with value of 478.25~MB/sec. GPU-SIFT uses 3,400 of the
3,584 available CUDA cores, running 2 pair image comparisons concurrently.
Note that GPU-SIFT throughput is almost double that of the CUDA-SIFT\@. This
shows that the overheads imposed by the CUDA Multi-Process Service (MPS) is
negligible for our implementation.

Fig.~\ref{fig:throughout} shows that GPU throughput is invariant to image
size. Increasing the image size increases the amount of data processed by the
GPU or CPU per second, bounded by the available GPU or CPU bandwidth. Note
that the error bars for the GPU implementations are smaller than those of the
CPU implementation. This is likely due to the efficiency of the CUDA
framework and the absence of competing processes on the GPU subsystem.

\begin{figure}%[ht!]
    \centering
    \begin{subfigure}{0.45\textwidth}
    \includegraphics[width=\linewidth]{figures/throughout.pdf}
    \caption{}\label{fig:throughout}
    \end{subfigure}
    ~
    \begin{subfigure}{0.45\textwidth}
    \includegraphics[width=\linewidth]{figures/memory.pdf}
    \caption{}\label{fig:memory}
    \end{subfigure}
    \caption{(a) The throughput of CPU-SIFT, CUDA-SIFT and GPU-SIFT as a function
	of image size in Megabytes. (b) Memory consumption of CPU-SIFT, CUDA-SIFT
	and GPU-SIFT as a function of tile size.}
\end{figure}

% ---------------------------------------------------------------------------
\subsection{Memory consumption}

We measure the memory consumption of CPU-SIFT, CUDA-SIFT and GPU-SIFT as the
amount of physical memory a particular program utilizes at runtime.
Fig.~\ref{fig:memory} shows the total memory consumption of CPU-SIFT,
GPU-SIFT and CUDA-SIFT for pairs of 2,000$^2$~px, 3,000$^2$~px, 4,000$^2$~px
and 5,000$^2$~px tiles. The memory usage includes tile reading and the SIFT
detecting, extracting, and matching of features.

For the largest tile of 5,000$^2$~px, CPU-SIFT consumes 24.67~GB of memory,
almost five times higher than CUDA-SIFT and GPU-SIFT which consume 8.05~GB
and 8.08~GB respectively. The minimal difference in memory consumption of
GPU-SIFT compared to CUDA-SIFT account for the acquisition of GeoTIFF images
and the use of CUDA MPS\@. This shows the minimal memory overhead that these
features require and therefore the minimal cost of doubling the throughput of
GPU-SIFT\@.

% ---------------------------------------------------------------------------
\subsection{Numbers of Matched points}

We measure the efficiency of each SIFT implementation in terms of the number
of matching points between a pair of images. We picked a pair of images for
which 16,850 true positive matches have been previously identified and
validated. We applied CPU-SIFT, GPU-SIFT and CUDA-SIFT on the pair of images
with different tile sizes to measure: (1) the number of matches that the
three implementations can detect; and (2) validate the assumption that the
tile size can affect the number of matches.

To measure the accuracy of both implementations we repeat the experiments up
to 75 times, using the same satellite image with tile sizes of 2,000$^2$~px,
3,000$^2$~px, 4,000$^2$~px and 5,000$^2$~px. Fig.~\ref{fig:accuracy} shows
that the number of matched points detected by CPU-SIFT is more than those
detected by GPU-SIFT and CUDA-SIFT\@. For 5,000$^2$~px tiles, CUDA-SIFT
returns 13,500 matches out of the existing 16,850 with an accuracy of
80.11\%. This is about 5.92\% more than GPU-SIFT, and 8.97\% more than
CUDA-SIFT\@. GPU-SIFT, plotted in green, returns 12,500 matches with an
accuracy of 74.18\%, while CUDA-SIFT, plotted in orange, returns 9,500
matches with an accuracy of 56.81\%.

\begin{figure}[ht!]
	\centering
	\begin{subfigure}{0.45\textwidth}
		\includegraphics[width=\linewidth]{figures/accuracy.pdf}
		\caption{}
		\label{fig:accuracy}
	\end{subfigure}
	~
	\begin{subfigure}{0.45\textwidth}
		\includegraphics[width=\linewidth]{figures/correct_matches.pdf}
		\caption{}
		\label{fig:correct_matches}
	\end{subfigure}
	\caption{shows the matching accuracy (a) and the total number of correct
	correspondences (b) found with GPU-SIFT, CUDA-SIFT and CPU-SIFT for
	well-known satellite image as a function of tile
	size.}\label{fig:accuracy_level}
\end{figure}

CPU-SIFT error bars shown in Fig.~\ref{fig:accuracy} are larger than those of
CUDA-SIFT and GPU-SIFT\@. It is unclear why CPU-SIFT is inconsistent in terms
of the number of matches and accuracy but, while in absolute terms it is the
implementation that can reach the highest number of matches, on average
GPU-SIFT with contrast enhancement offer a more reliable performance.

It's worth mentioning that CPU-SIFT and GPU-SIFT apply contrast enhancement
to both source and target images before processing them, while CUDA-SIFT does
not apply any contrast enhancement. Enhancing the level of contrast of an
image can increase the numbers of detected features and as a result, it
directly increases the number of matches between both images.

